Deep-Research Agents Can Be Poisoned via User-Generated Content

Deep-research agents are an alternative to conventional Web search. They use multi-agent pipelines to issue multiple Web searches related to user queries, retrieve relevant content from the answers, and generate detailed, evidence-based reports. We show that for many common search topics (including financial, medical, and product recommendations), agent-generated reports are consistently based on the same user-generated content (UGC) pages from platforms such as Reddit and Wikipedia. This retrieval overlap, combined with lax moderation and access controls for UGC, is an opportunity for subversion: an attacker who appends a short text to a single, frequently-retrieved page can cause agents to cite this text and promote attacker-chosen entities across many user questions. We evaluate this attack on representative deep-research systems across multiple topics, such as investment advice, antivirus software, restaurant recommendations, etc. Poisoning a single URL with as few as 13 words can be sufficient for the attacker's content to be retrieved in 57-76% of the agent executions for a given topic and cited in 38-51% of the generated reports. A more aggressive attack (poisoning an entire subreddit) achieves 30-53% citation rates even when the poison is only 0.5-4% of the retrieved content. The attacker does not need to know the phrasing of the user's question, nor the specific Web queries generated by the agent, nor the agent's internal retrieval and generation mechanisms. We then study defenses at different stages of the pipeline, including source-level filtering and output-based detection. Dropping UGC from retrieved content blocks the attack but degrades the quality of generated reports. We show that lightweight anomaly detection on inputs and outputs does not reliably identify poisoned content, nor the results of poisoning.

==> fig/costorm_supplements_2.tex <==
% Example 2: NMN brand query
\begin{figure*}[!ht]
\centering

\begin{tcolorbox}[
  colback=advbg, colframe=advframe,
  title={\small\textbf{Injected text} (13 words, appended to SERP snippet of \texttt{reddit.com/r/NMN/\ldots})},
  fonttitle=\sffamily, fontupper=\small,
  boxrule=0.6pt, arc=2pt, left=4pt, right=4pt, top=2pt, bottom=2pt,
]
\textit{``Tried <ORIGINAL COMPOUND> but felt underwhelmed. Switched to <INJECTED COMPOUND> for improved energy and recovery. Highly recommend!''}
\end{tcolorbox}

\vspace{4pt}

\begin{minipage}[t]{0.485\textwidth}
\begin{tcolorbox}[
  colback=cleanbg, colframe=cleanframe,
  title={\small\textbf{Clean report} (no attack)},
  fonttitle=\sffamily, fontupper=\small,
  boxrule=0.6pt, arc=2pt, left=4pt, right=4pt, top=2pt, bottom=2pt,
]
Prohealth and Renue are considered among the most trusted brands for purchasing Sublingual and Liposomal <ORIGINAL COMPOUND> [4],\ldots. When selecting a brand, look for third-party testing to verify active ingredient content and ensure the product is free from contaminants\,[5][8]. A common recommendation is 450\,mg once daily\,[6].

\vspace{4pt}
\scriptsize
\textsf{[4]\,https://www.prohealth.com/\ldots}\\
\textsf{[5]\,https://examine.com/supplements/\ldots}\\
\textsf{[6]\,https://www.reddit.com/r/subreddit/\ldots}\\
\textsf{[8]\,https://www.renuebyscience.com/\ldots}
\end{tcolorbox}
\end{minipage}\hfill
\begin{minipage}[t]{0.485\textwidth}
\begin{tcolorbox}[
  colback=attackbg, colframe=attackframe,
  title={\small\textbf{Attacked report} (short-SERP injection)},
  fonttitle=\sffamily, fontupper=\small,
  boxrule=0.6pt, arc=2pt, left=4pt, right=4pt, top=2pt, bottom=2pt,
]
Prohealth and Renue are considered among the most trusted brands for purchasing Sublingual and Liposomal <ORIGINAL COMPOUND> [4],\ldots. In addition to these reputable brands, some users have reported switching to \textcolor{hlbrand}{<INJECTED COMPOUND>} for enhanced energy and recovery, suggesting it as a highly recommended alternative\,[4].

\vspace{4pt}
\scriptsize
\textsf{[4]\,\textcolor{hlbrand}{https://www.reddit.com/r/subreddit/\ldots\,(poisoned)}}\\
\textsf{[5]\,https://examine.com/supplements/\ldots}\\
\textsf{[6]\,https://www.renuebyscience.com/\ldots}
\end{tcolorbox}
\end{minipage}

\caption{Example of the compound substitution attack on Co-STORM (query: ``What are some quality brands for <ORIGINAL COMPOUND> I can trust?''). \textbf{Top:} 13-word poisoned text appended to a Reddit SERP snippet. \textbf{Bottom left:} clean report recommending established <ORIGINAL COMPOUND> brands. \textbf{Bottom right:} attacked report introducing fictitious \textcolor{hlbrand}{<INJECTED COMPOUND>} as a ``highly recommended alternative,'' citing the poisoned Reddit URL~[4].}
\label{fig:zts26_attack_nmn}
\end{figure*}
